Targeted Adversarial Attacks on Generalizable Neural Radiance Fields

Neural Radiance Fields (NeRFs) have recently emerged as a powerful tool for 3D scene representation and rendering. These data-driven models can learn to synthesize high-quality images from sparse 2D observations, enabling realistic and interactive scene reconstructions. However, the growing usage of NeRFs in critical applications such as augmented reality, robotics, and virtual environments could be threatened by adversarial attacks. In this paper we present how generalizable NeRFs can be attacked by both low-intensity adversarial attacks and adversarial patches, where the later could be robust enough to be used in real world applications. We also demonstrate targeted attacks, where a specific, predefined output scene is generated by these attack with success.

==> reviews.tex <==

1. Summary
In this paper, the authors study the robustness of Generalizable Neural Radiance Fields (Gen-Nerf), from the perspective of inducing the model to output a specified output image. Thus, the paper explores the use of adversarial perturbations on source images of different views to fool the NERF model in a targeted manner.
2. Strengths
1) The paper considers an interesting setting of analysing the adversarial vulnerability of Gen-NERF to targeted adversarial attacks, as opposed to prior works that focus on the untargeted setting.
2) The attacks are seen to be effective in general, though the quantitative metrics used could be improved in being more comprehensive.
3) The paper shows that the model is sensitive to both low-intensity attacks (Lp constrained attacks) and patch-based adversaries.


3. Weaknesses
1) The images considered as target outputs could have been set to be highly different from the original output, since the constraint on the size of the perturbation applied is only with respect to the input-source images. Thus, it would constitute a much more "problematic" case wherein the induced output is significantly different, rather than small modifications.
BANDI-
Low priority



2) The similarity of the produced output image and target image could have been better characterized by including more diverse metrics, and not just the L2-metric since is dependent on the image resolution etc. Other metrics such as MSE, and even perceptual measures such as SSIM or LPIPS could be included to better understand the nature of the outputs produced.
PSNR, SSIM, LPIPS
BANDI
High priority



3) The paper could have included other analyses on the transferability of the adversarial perturbations in being effective at nearby viewing angles as well, that is, whether the attack is effective in some neighbourhood-view of the target image as well.
Több output kép legyen és nézzük meg,hogy ott tudunk e a pontfelhőbe objetumot tenni vagy sem...
BANDI
Low priority...
-Esetleg nézzük meg,hogy kcis más szeögből megmarad-e a maci...


4) The exact applicability of the attack could be perhaps motivated better, since it is not completely clear what kind of security risks such attacks pose in practice for NERF models.
BANDI/CSABA
Ha isemerem a NERF-et és ismerem a környezetet, akkor meg tudom támadni úgy,hogy tetszőleges objektumok ott legyen...Ha...
Erre váalszoljunk a szövegben 

4. Recommendation
Weak Accept
5. Justifications for the recommendation
The paper studies an interesting area of targeted attacks on Gen-Nerf using both Lp and Patch based adversaries. The evaluation and a few other aspects could be improved as mentioned in the Weaknesses section.





1. Summary
NeRF is a major way to represent 3D scene and rendering novel views. This paper studied a specific variant of NeRF that based on generalization, the method did not study how to work on NeRF with individual scene optimization. The paper shows effectiveness in attack gen-NeRF, with two types of attack. Visualizations and numerical results show the effectiveness of the approach.
2. Strengths
1. Interesting problem. This is the first work, to the reviewer's knowledge, that creates adversarial attack for neural radiance field.

2. Figure 2 clearly shows that the proposed attack can modify and delete objects in the image.

3. Ablation study on number of source views attacked are shown.


3. Weaknesses
1. Attack method limits to a specific family of neural radiance fields. The method, to the reviewers understanding, cannot generalize to NeRF, because NeRF train field for each scene, for many steps, and the proposed method cannot attack that. It would be great if the author can show it can be modified to attack NeRF, since that is the most standard approach.
CSABA
Erre csak vaálszojlunk, hogy tot a betanított modell-t kéne piszkálni...és az nem nagoyn hanszálható a gykaorlatban.

2. Figure 1 is a duplicate from the architecture of the original paper. The author should show where the attack happens in the figure. Otherwise this figure adds no information.
- CSABA
Egész doboz kimehet középről és oda mehet egy GENNERf doboz ...és valahogy a gradienst jó lenne jelezni.
Egy msái kverituális kép, amin szerep la patch...vagy módosítás


3. Attack is whitebox, assume gen-NeRF family, which is not very realistic.
Nem érzem fontosnak
Irdolaomban szinte mindenki whitebox-al foglalkozik... , azért mert:
Elvileg megodlható, viszont rengeteg futtatás igényel.
itt az volta  fúkusz,hogy lehet-e ilyet cisnálni...

BANDI
Minor:
L129: Typo.


4. Recommendation
Borderline Accept
5. Justifications for the recommendation
The paper studies an interesting problem, can attack a specific type of neural radiance model. Yet the quality of the writing and content needs significant improving.


Megnézni azt,hogy a 3D struktúra minél jobban változzon, de a renderelt kép meg ne változzon egyáltalán.
és erre csinálni attack-ot
